Backdoor Graph Condensation

Graph condensation has recently emerged as a prevalent technique to improve the training efficiency for graph neural networks (GNNs). It condenses a large graph into a small one such that a GNN trained on this small synthetic graph can achieve comparable performance to a GNN trained on the large graph. However, while existing graph condensation studies mainly focus on the best trade-off between graph size and the GNNs' performance (model utility), they overlook the security issues of graph condensation. To bridge this gap, we first explore backdoor attack against the GNNs trained on the condensed graphs. We introduce an effective backdoor attack against graph condensation, termed BGC. This attack aims to (1) preserve the condensed graph quality despite trigger injection, and (2) ensure trigger efficacy through the condensation process, achieving a high attack success rate. Specifically, BGC consistently updates triggers during condensation and targets representative nodes for poisoning. Extensive experiments demonstrate the effectiveness of our attack. BGC achieves a high attack success rate (close to 1.0) and good model utility in all cases. Furthermore, the results against multiple defense methods demonstrate BGC's resilience under their defenses. Finally, we analyze the key hyperparameters that influence the attack performance. Our code is available at: https://github.com/JiahaoWuGit/BGC.

==> sections/experiment-results/compare-with-baselines/on-DC-graph.tex <==
% \begin{subtable}\centering
\subcaptionbox{Condensation Method: DC-Graph\label{subtab:DC-Graph-compare-with-baselines}}{
    \begin{tabular}{c|c|c|cc|cc|cc}
    \hline
     & {\color[HTML]{1F1F1F} }       &              & \multicolumn{2}{c|}{GTA}    & \multicolumn{2}{c|}{DOORPING-Graph} & \multicolumn{2}{c}{BGC}                      \\ \cline{4-9} 
    \multirow{-2}{*}{Datasets} &
      \multirow{-2}{*}{{\color[HTML]{1F1F1F} Ratio (r)}} &
      \multirow{-2}{*}{CMA (\%)} &
      CTA (\%) &
      ASR (\%) &
      CTA (\%) &
      ASR (\%) &
      CTA (\%) &
      ASR (\%) \\ \hline
     & {\color[HTML]{1F1F1F} 1.30\%} & 75.17 (0.65) & 68.97 (2.05) & 100.0 (0.00) & 66.10 (0.17)     & 100.0 (0.00)     & \textbf{75.90 (0.94)} & \textbf{100.0 (0.00)} \\
     & {\color[HTML]{1F1F1F} 2.60\%} & 75.97 (0.61) & 72.30 (0.75) & 100.0 (0.00) & 73.50 (0.96)     & 100.0 (0.00)     & \textbf{75.00 (0.51)} & \textbf{100.0 (0.00)} \\
    \multirow{-3}{*}{Cora} &
      {\color[HTML]{1F1F1F} 5.20\%} &
      78.30 (0.43) &
      75.93 (0.09) &
      100.0 (0.00) &
      76.00 (0.54) &
      100.0 (0.00) &
      \textbf{78.43 (0.31)} &
      \textbf{100.0 (0.00)} \\ \hline
     & {\color[HTML]{1F1F1F} 0.90\%} & 68.37 (0.90) & 65.90 (1.02) & 100.0 (0.00) & 66.90 (1.07)     & 100.0 (0.00)     & \textbf{70.27 (0.50)} & \textbf{100.0 (0.00)} \\
     & {\color[HTML]{1F1F1F} 1.80\%} & 69.10 (0.62) & 67.43 (0.87) & 100.0 (0.00) & 67.20 (0.57)     & 100.0 (0.00)     & \textbf{69.37 (0.94)} & \textbf{100.0 (0.00)} \\
    \multirow{-3}{*}{Citeseer} &
      {\color[HTML]{1F1F1F} 3.60\%} &
      70.23 (0.05) &
      67.03 (1.00) &
      100.0 (0.00) &
      67.50 (0.36) &
      100.0 (0.00) &
      \textbf{70.00 (0.22)} &
      \textbf{100.0 (0.00)} \\ \hline
     & {\color[HTML]{1F1F1F} 0.10\%} & 45.49 (0.43) & 45.09 (0.42) & 90.13 (0.57) & 45.20 (0.23)     & 91.05 (1.10)     & \textbf{46.48 (0.21)} & \textbf{99.98 (0.02)} \\
     & {\color[HTML]{1F1F1F} 0.50\%} & 46.37 (0.10) & 46.01 (0.05) & 89.83 (0.78) & 46.17 (0.11)     & 93.09 (2.35)     & \textbf{46.44 (0.13)} & \textbf{99.25 (0.85)} \\
    \multirow{-3}{*}{Flickr} &
      {\color[HTML]{1F1F1F} 1.00\%} &
      47.14 (0.03) &
      46.15 (0.12) &
      90.45 (0.44) &
      46.07 (0.07) &
      91.66 (0.83) &
      \textbf{46.77 (0.30)} &
      \textbf{99.11 (0.40)} \\ \hline
     & {\color[HTML]{1F1F1F} 0.05\%} & 85.88 (0.08) & 85.75 (0.58) & 90.32 (0.12) & 85.07 (0.30)     & 94.17 (1.62)     & \textbf{85.38 (0.42)} & \textbf{99.90 (0.03)} \\
     & {\color[HTML]{1F1F1F} 0.10\%} & 89.25 (0.21) & 88.87 (0.24) & 89.09 (0.94) & 88.46 (0.21)     & 90.01 (0.70)     & \textbf{89.14 (0.05)} & \textbf{99.93 (0.02)} \\
    \multirow{-3}{*}{Reddit} &
      {\color[HTML]{1F1F1F} 0.20\%} &
      91.15 (0.07) &
      90.07 (0.32) &
      89.62 (0.34) &
      90.24 (0.14) &
      91.21 (0.93) &
      \textbf{90.38 (0.42)} &
      \textbf{99.90 (0.03)} \\ \hline
    \end{tabular}
}
%     \label{subtab:DC-Graph-compare-with-baselines}
%     % \caption{With DC-Graph}
% \end{subtable}

==> sections/experiment-results/compare-with-baselines/on-GCond-X.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\subcaptionbox{Condensation Method: GCond-X\label{subtab:GCond-X-compare-with-baselines}}{
\begin{tabular}{c|c|c|cc|cc|cc}
\hline
 & {\color[HTML]{1F1F1F} }       &               & \multicolumn{2}{c|}{GTA}    & \multicolumn{2}{c|}{DOORPING-Graph}  & \multicolumn{2}{c}{BGC}                       \\ \cline{4-9} 
\multirow{-2}{*}{Datasets} &
  \multirow{-2}{*}{{\color[HTML]{1F1F1F} Ratio (r)}} &
  \multirow{-2}{*}{CMA (\%)} &
  CTA (\%) &
  ASR (\%) &
  CTA (\%) &
  ASR (\%) &
  CTA (\%) &
  ASR (\%) \\ \hline
 & {\color[HTML]{1F1F1F} 1.30\%} & 77.67 (0.59)  & 75.40 (1.85) & 89.00 (0.08) & 75.67 (0.74) & 100.0 (0.00)          & \textbf{76.30 (1.35)} & \textbf{100.0 (0.00)} \\
 & {\color[HTML]{1F1F1F} 2.60\%} & 78.70 (0.90)  & 79.27 (0.25) & 88.57 (0.21) & 79.63 (0.52) & 100.0 (0.00)          & \textbf{78.10 (0.71)} & \textbf{100.0 (0.00)} \\
\multirow{-3}{*}{Cora} &
  {\color[HTML]{1F1F1F} 5.20\%} &
  80.40 (1.28) &
  80.63 (0.82) &
  93.13 (0.05) &
  81.47 (0.25) &
  100.0 (0.00) &
  \textbf{79.40 (0.36)} &
  \textbf{100.0 (0.00)} \\ \hline
 & {\color[HTML]{1F1F1F} 0.90\%} & 73. 76 (0.21) & 69.00 (1.77) & 89.47 (0.05) & 55.47 (0.79) & 92.00 (0.48)          & \textbf{73.03 (0.50)} & \textbf{100.0 (0.00)} \\
 & {\color[HTML]{1F1F1F} 1.80\%} & 72.07 (0.61)  & 72.00 (0.22) & 88.63 (0.26) & 63.63 (0.49) & 96.67 (0.62)          & \textbf{72.40 (0.57)} & \textbf{100.0 (0.00)} \\
\multirow{-3}{*}{Citeseer} &
  {\color[HTML]{1F1F1F} 3.60\%} &
  72.16 (0.00) &
  69.23 (1.32) &
  85.13 (0.09) &
  55.47 (0.97) &
  90.55 (1.45) &
  \textbf{72.13 (0.83)} &
  \textbf{100.0 (0.00)} \\ \hline
 & {\color[HTML]{1F1F1F} 0.10\%} & 45.60 (0.80)  & 45.78 (0.22) & 87.10 (0.33) & 45.79 (0.05) & \textbf{100.0 (0.00)} & \textbf{46.15 (0.47)} & \textbf{98.26 (2.19)} \\
 & {\color[HTML]{1F1F1F} 0.50\%} & 46.68 (0.20)  & 45.21 (0.16) & 83.44 (3.32) & 45.09 (0.12) & \textbf{100.0 (0.00)} & \textbf{46.21 (0.44)} & \textbf{99.58 (0.55)} \\
\multirow{-3}{*}{Flickr} &
  {\color[HTML]{1F1F1F} 1.00\%} &
  45.74 (0.31) &
  45.11 (0.15) &
  81.29 (0.24) &
  45.12 (0.22) &
  \textbf{100.0 (0.00)} &
  \textbf{45.62 (0.17)} &
  \textbf{95.51 (1.69)} \\ \hline
 & {\color[HTML]{1F1F1F} 0.05\%} & 87.09 (0.10)  & 86.48 (0.43) & 90.08 (1.20) & 87.41 (0.63) & 91.40 (1.98)          & \textbf{87.47 (0.21)} & \textbf{99.89 (0.15)} \\
 & {\color[HTML]{1F1F1F} 0.10\%} & 88.42 (0.47)  & 87.34 (0.12) & 95.23 (0.47) & 88.44 (0.19) & 92.81 (0.21)          & \textbf{89.14 (0.51)} & \textbf{99.78 (0.30)} \\
\multirow{-3}{*}{Reddit} &
  {\color[HTML]{1F1F1F} 0.20\%} &
  89.96 (0.14) &
  88.70 (0.22) &
  96.52 (0.13) &
  89.30 (0.23) &
  94.12 (0.43) &
  \textbf{90.09 (0.21)} &
  \textbf{97.60 (2.42)} \\ \hline
\end{tabular}
}

==> sections/experiment-results/compare-with-baselines/on-GCond.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\subcaptionbox{Condensation Method: GCond\label{subtab:GCond-compare-with-baselines}}{
\begin{tabular}{c|c|c|cc|cc|cc}
\hline
\multirow{2}{*}{Datasets} &
  \multirow{2}{*}{Ratio (r)} &
  \multirow{2}{*}{CMA (\%)} &
  \multicolumn{2}{c|}{GTA} &
  \multicolumn{2}{c|}{DOORPING-Graph} &
  \multicolumn{2}{c}{BGC} \\ \cline{4-9} 
                        &        &              & CTA (\%)     & ASR (\%)     & CTA (\%)     & ASR (\%)     & CTA (\%)              & ASR (\%)              \\ \hline
\multirow{3}{*}{Cora}   & 1.30\% & 81.33 (0.62) & 80.13 (0.56) & 100.0 (0.00) & 80.87 (0.73) & 100.0 (0.00) & \textbf{81.23 (0.24)} & \textbf{100.0 (0.00)} \\
                        & 2.60\% & 81.27 (0.33) & 79.93 (0.29) & 100.0 (0.00) & 79.77 (0.33) & 100.0 (0.00) & \textbf{80.67 (0.52)} & \textbf{100.0 (0.00)} \\
                        & 5.20\% & 80.53 (0.73) & 78.33 (0.71) & 100.0 (0.00) & 80.03 (0.42) & 100.0 (0.00) & \textbf{80.70 (0.50)} & \textbf{100.0 (0.00)} \\ \hline
\multirow{3}{*}{Citeseer} &
  0.90\% &
  71.43 (0.33) &
  69.30 (0.59) &
  100.0 (0.00) &
  54.60 (0.08) &
  100.0 (0.00) &
  \textbf{71.57 (1.32)} &
  \textbf{100.0 (0.00)} \\
                        & 1.80\% & 72.03 (0.17) & 68.53 (0.29) & 100.0 (0.00) & 69.30 (0.80) & 100.0 (0.00) & \textbf{71.03 (0.09)} & \textbf{100.0 (0.00)} \\
                        & 3.60\% & 71.20 (0.70) & 69.07 (1.40) & 100.0 (0.00) & 68.03 (0.50) & 100.0 (0.00) & \textbf{70.60 (0.51)} & \textbf{100.0 (0.00)} \\ \hline
\multirow{3}{*}{Flickr} & 0.10\% & 46.85 (0.10) & 46.00 (0.07) & 92.07 (0.19) & 46.01 (0.16) & 93.16 (0.03) & \textbf{46.54 (0.08)} & \textbf{99.83 (0.07)} \\
                        & 0.50\% & 46.62 (0.53) & 46.32 (0.30) & 96.53 (0.12) & 46.50 (0.08) & 95.33 (1.31) & \textbf{47.15 (0.08)} & \textbf{99.97 (0.02)} \\
                        & 1.00\% & 46.91 (0.41) & 45.82 (0.36) & 94.57 (1.63) & 45.69 (0.32) & 93.54 (2.13) & \textbf{46.84 (0.09)} & \textbf{99.77 (0.06)} \\ \hline
\multirow{3}{*}{Reddit} & 0.05\% & 88.86 (0.06) & 82.14 (0.26) & 93.33 (2.61) & 87.95 (0.39) & 92.00 (2.08) & \textbf{88.50 (0.27)} & \textbf{99.84 (0.14)} \\
                        & 0.10\% & 89.20 (0.13) & 83.10 (1.28) & 96.25 (0.18) & 89.71 (0.28) & 98.33 (0.44) & \textbf{90.37 (0.22)} & \textbf{99.99 (0.01)} \\
                        & 0.20\% & 90.10 (0.26) & 83.03 (0.53) & 97.80 (0.22) & 90.28 (0.30) & 96.16 (3.18) & \textbf{90.40 (0.41)} & \textbf{99.06 (0.91)} \\ \hline
\end{tabular}
}

==> sections/experiment-results/compare-with-baselines/on-SNTK.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\subcaptionbox{Condensation Method: SNTK\label{subtab:SNTK-compare-with-baselines}}{
\begin{tabular}{c|c|c|cc|cc|cc}
\hline
 &
  {\color[HTML]{1F1F1F} } &
   &
  \multicolumn{2}{c|}{GTA} &
  \multicolumn{2}{c|}{DOORPING-Graph} &
  \multicolumn{2}{c}{BGC} \\ \cline{4-9} 
\multirow{-2}{*}{Datasets} &
  \multirow{-2}{*}{{\color[HTML]{1F1F1F} Ratio (r)}} &
  \multirow{-2}{*}{CMA (\%)} &
  CTA (\%) &
  ASR (\%) &
  CTA (\%) &
  ASR (\%) &
  CTA (\%) &
  ASR (\%) \\ \hline
 &
  {\color[HTML]{1F1F1F} 1.30\%} &
  81.24 (0.50) &
  73.18 (2.03) &
  82.33 (1.34) &
  71.80 (14.21) &
  88.80 (0.90) &
  \textbf{79.73 (1.40)} &
  \textbf{98.30 (1.53)} \\
 &
  {\color[HTML]{1F1F1F} 2.60\%} &
  80.50 (0.70) &
  77.66 (0.40) &
  85.22 (0.94) &
  79.30 (0.62) &
  87.50 (1.07) &
  \textbf{79.10 (1.04)} &
  \textbf{99.77 (0.15)} \\
\multirow{-3}{*}{Cora} &
  {\color[HTML]{1F1F1F} 5.20\%} &
  80.12 (0.32) &
  78.01 (0.16) &
  82.11 (0.14) &
  79.10 (0.63) &
  81.30 (1.27) &
  \textbf{79.67 (0.42)} &
  \textbf{98.13 (1.65)} \\ \hline
 &
  {\color[HTML]{1F1F1F} 0.90\%} &
  60.68 (1.04) &
  59.02 (0.14) &
  85.46 (0.26) &
  58.57 (4.22) &
  86.80 (0.67) &
  \textbf{60.20 (3.64)} &
  \textbf{100.0 (0.00)} \\
 &
  {\color[HTML]{1F1F1F} 1.80\%} &
  62.33 (2.06) &
  62.39 (1.33) &
  85.18 (0.91) &
  62.10 (1.05) &
  85.93 (1.31) &
  \textbf{63.03 (2.64)} &
  \textbf{100.0 (0.00)} \\
\multirow{-3}{*}{Citeseer} &
  {\color[HTML]{1F1F1F} 3.60\%} &
  63.44 (1.30) &
  61.99 (0.78) &
  86.54 (0.25) &
  62.40 (1.55) &
  87.33 (0.89) &
  \textbf{63.37 (2.06)} &
  \textbf{100.0 (0.00)} \\ \hline
 &
  {\color[HTML]{1F1F1F} 0.10\%} &
  46.10 (0.10) &
  45.10 (0.67) &
  86.15 (1.23) &
  45.80 (0.13) &
  \textbf{84.26 (0.24)} &
  \textbf{46.32 (0.09)} &
  \textbf{99.98 (0.00)} \\
 &
  {\color[HTML]{1F1F1F} 0.50\%} &
  46.23 (0.10) &
  45.79 (0.14) &
  86.38 (0.58) &
  46.02 (0.12) &
  \textbf{85.59 (1.62)} &
  \textbf{46.02 (0.21)} &
  \textbf{99.98 (0.00)} \\
\multirow{-3}{*}{Flickr} &
  {\color[HTML]{1F1F1F} 1.00\%} &
  46.01 (0.20) &
  45.19 (0.11) &
  86.35 (0.37) &
  45.99 (0.08) &
  \textbf{85.46 (0.86)} &
  \textbf{45.50 (0.06)} &
  \textbf{99.98 (0.00)} \\ \hline
 &
  {\color[HTML]{1F1F1F} 0.05\%} &
  OOM &
  OOM &
  OOM &
  OOM &
  OOM &
  \textbf{OOM} &
  \textbf{OOM} \\
 &
  {\color[HTML]{1F1F1F} 0.10\%} &
  OOM &
  OOM &
  OOM &
  OOM &
  OOM &
  \textbf{OOM} &
  \textbf{OOM} \\
\multirow{-3}{*}{Reddit} &
  {\color[HTML]{1F1F1F} 0.20\%} &
  OOM &
  OOM &
  OOM &
  OOM &
  OOM &
  \textbf{OOM} &
  \textbf{OOM} \\ \hline
\end{tabular}
}

==> sections/experiment-results/random-select-ablation/dc-graph/sub-figure-main-4datasets.tex <==
% \begin{subfigure}{1.0\linewidth}
        \begin{tabular}{cccc}
            %CTA DC-graph
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/cora-CTA-DC-graph}
                }
                % \caption{\label{subfig:select-ablation-cora-cta-dc-graph}With DC-Graph on Cora}
            \end{subfigure}
            &
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/citeseer-CTA-DC-graph}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/flickr-CTA-DC-graph}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/reddit-CTA-DC-graph}
                }
            \end{subfigure} 
            \\
            
            %ASR DC-graph
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/cora-ASR-DC-graph}
                }
                % \caption{\label{subfig:select-ablation-cora-cta-dc-graph}With DC-Graph on Cora}
            \end{subfigure}
            &
            % \begin{subfigure}{0.23\linewidth}
            %     \resizebox{1.0\linewidth}{!}{
            %         \input{sections/experiment-results/random-select-ablation/dc-graph/cora-ASR-DC-graph}
            %     }
            %     % \caption{\label{subfig:select-ablation-cora-cta-dc-graph}With DC-Graph on Cora}
            % \end{subfigure}
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/citeseer-ASR-DC-graph-new}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/flickr-ASR-DC-graph}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.23\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \input{sections/experiment-results/random-select-ablation/dc-graph/reddit-ASR-DC-graph}
                }
            \end{subfigure}
        \end{tabular}
        % \caption{Condensation Method: DC-Graph.}
    % \end{subfigure}

==> sections/experiment-results/random-select-ablation/figures/sub-fig-dc-graph-main.tex <==
\begin{subfigure}{1.0\linewidth}
        \centering
        \begin{tabular}{cccc}
            % CTA DC-graph
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-cta-cora.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-cta-citeseer.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-cta-flickr.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-cta-reddit.png}
                }
            \end{subfigure} 
            \\
            
            %ASR DC-graph
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-asr-cora.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-asr-citeseer.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-asr-flickr.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/DC-graph/DC-graph-asr-reddit.png}
                }
            \end{subfigure}
            
        \end{tabular}
        \caption{Condensation Method: DC-Graph.}
    \end{subfigure}

==> sections/experiment-results/random-select-ablation/figures/sub-fig-gcond-main.tex <==
\begin{subfigure}{1.0\linewidth}
        \centering
        \begin{tabular}{cccc}
            % CTA GCond
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-cta-cora.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-cta-citeseer.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-cta-flickr.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-cta-reddit.png}
                }
            \end{subfigure} 
            \\
            
            %ASR GCond
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-asr-cora.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-asr-citeseer.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-asr-flickr.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond/GCond-asr-reddit.png}
                }
            \end{subfigure}
            
        \end{tabular}
        \caption{Condensation Method: GCond.}
    \end{subfigure}

==> sections/experiment-results/random-select-ablation/figures/sub-fig-gcond-x-main.tex <==
\begin{subfigure}{1.0\linewidth}
        \centering
        \begin{tabular}{cccc}
            % CTA GCond-X
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-cta-cora.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-cta-citeseer.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-cta-flickr.png}
                }
            \end{subfigure} 
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-cta-reddit.png}
                }
            \end{subfigure} 
            \\
            
            %ASR GCond-X
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-asr-cora.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-asr-citeseer.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-asr-flickr.png}
                }
            \end{subfigure}
            &
            \begin{subfigure}{0.2\linewidth}
                \resizebox{1.0\linewidth}{!}{
                    \includegraphics{sections/experiment-results/random-select-ablation/figures/GCond-X/GCond-X-asr-reddit.png}
                }
            \end{subfigure}
            
        \end{tabular}
        \caption{Condensation Method: GCond-X.}
    \end{subfigure}
